MINLP in Transmission Expansion Planning

Transmission expansion planning requires forecasts of demand for electric power and a model of the underlying physics, i.e., power flows. We present three approaches to deriving exact solutions to the transmission expansion planning problem in the alternating-current model, for a given load.

==> tables3/case2_01_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             &  DC VM &   VA   & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &   VA   \\ \hline 
   Obj / T   & 700.00 &  0.02  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 & 877.78 &  0.25  \\ \hline 
 RMSE / MAPE &  18.25 &  -0.09 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  9.73  &  -0.04 \\ \hline 
      B1     &  1.00  &  0.00  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.95  &  0.00  \\ \hline 
      B2     &  1.00  & -40.11 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  1.05  & -57.14 \\ \hline 
\end{tabular}


==> tables3/case2_10_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             &  DC VM &   VA   & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &   VA   \\ \hline 
   Obj / T   & 700.00 &  0.02  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 & 838.46 &  0.21  \\ \hline 
 RMSE / MAPE &  6.45  &  -0.06 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  2.76  &  -0.02 \\ \hline 
      B1     &  1.00  &  0.00  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.99  &  0.00  \\ \hline 
      B2     &  1.00  & -20.05 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  1.05  & -27.43 \\ \hline 
\end{tabular}


==> tables3/case2_11_convergence.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|}\hline
 r & rows & cols. &  nnz.  &  time  & $y_1$ & $y_2$ \\ \hline 
 1 &  100 &  547  &   594  &  4.42  &  0.64 &  0.64 \\ \hline 
 2 &  787 &  6355 &  10123 &  9.92  &  0.74 &  0.80 \\ \hline 
 3 & 6105 & 92245 & 163314 & 186.97 &  0.92 &  0.93 \\ \hline 
\end{tabular}


==> tables3/case2_11_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             &  DC VM &   VA   & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &   VA   \\ \hline 
   Obj / T   & 700.00 &  0.02  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 & 800.00 &  0.21  \\ \hline 
 RMSE / MAPE &  3.35  &  0.11  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  5.72  &  -0.03 \\ \hline 
      B1     &  1.00  &  0.00  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  1.04  &  -0.00 \\ \hline 
      B2     &  1.00  & -13.37 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  1.05  & -18.12 \\ \hline 
\end{tabular}


==> tables3/case2_comparison.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
 r & rows & cols. & nnz. & time & obj. &  err. & $y_1$ & r & rows & cols. & nnz. & time & obj. &  err. & $y_1$ & r & rows & cols. & nnz. & time &  obj. &  err. & $y_1$ & r & rows & cols. & nnz. & time &  obj. &  err. & $y_1$ \\ \hline 
 1 &  104 &  662  & 1059 & 0.24 & 0.00 & -3.50 &  0.00 & 1 &  125 &  707  & 1148 & 0.27 & 0.00 & -3.50 &  0.00 & 1 &  70  &  311  &  336 & 0.61 & -0.00 & -3.70 &  0.00 & 1 &  71  &  311  &  336 & 0.59 & -0.00 & -3.68 &  0.00 \\ \hline 
 2 &  104 &  662  & 1059 & 0.22 & 0.00 & -3.50 &  0.00 & 2 &  125 &  707  & 1148 & 0.29 & 0.00 & -3.50 &  0.00 & 2 &  489 &  3305 & 5425 & 2.25 &  0.00 & -3.50 &  0.00 & 2 &  525 &  3370 & 5550 & 3.48 &  0.00 & -3.49 &  0.00 \\ \hline 
\end{tabular}


==> tables3/case2m_comparison1.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
 r & rows &  cols. &  nnz.  &  time &  obj.  &  err. &  $y_1$  & r & rows &  cols. &  nnz.  &  time  &  obj.  &  err. &  $y_1$  \\ \hline 
 1 &  104 &   626  &  1010  &  2.29 & 877.78 & -3.50 & 0.00000 & 1 &  120 &   628  &  1034  &  0.55  & 877.78 & -3.50 & 0.00000 \\ \hline 
 2 &  104 &   626  &  1010  &  0.42 & 877.78 & -3.50 & 0.00000 & 2 &  120 &   628  &  1034  &  0.49  & 877.78 & -3.50 & 0.00000 \\ \hline 
 3 &  335 &  5190  &  10791 &  1.47 & 877.78 & -3.50 & 0.00000 & 3 &  456 &  5967  &  13343 &  2.22  & 877.78 & -3.50 & 0.00000 \\ \hline 
 4 &  824 &  29227 &  70364 & 11.93 & 877.78 & -3.50 & 0.00000 & 4 & 1281 &  37981 & 108087 &  19.30 & 877.78 & -3.50 & 0.00000 \\ \hline 
 5 & 1715 & 124568 & 326630 & 68.52 & 877.78 & -3.50 & 0.00000 & 5 & 2997 & 183361 & 624152 & 214.05 & 877.78 & -3.50 & 0.00000 \\ \hline 
\end{tabular}


==> tables3/case2m_comparison2.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
 r &  rows &  cols.  &   nnz.  &   time   &  obj.  &  err. &  $y_1$  & r &  rows &  cols.  &   nnz.  &   time   &  obj.  &  err. &  $y_1$  \\ \hline 
 1 &   70  &   310   &   335   &   1.23   &  -0.00 & -3.73 & 0.00000 & 1 &   71  &   310   &   335   &   1.07   &  -0.00 & -3.81 & 0.00000 \\ \hline 
 2 &  489  &   3241  &   5328  &   4.38   &  0.00  & -3.50 & 0.00001 & 2 &  447  &   2919  &   5036  &   5.57   &  0.00  & -3.50 & 0.00000 \\ \hline 
 0 &   0   &    0    &    0    &   0.00   &  0.00  &  0.00 & 0.00000 & 3 &  2747 &  35334  &  73644  &   54.96  &  0.40  & -3.50 & 0.00255 \\ \hline 
 4 & 11219 &  299458 &  652591 &  1886.08 &  97.29 & -3.50 & 0.91859 & 4 & 11243 &  286700 &  689785 &  1913.36 &  44.57 & -3.50 & 0.39360 \\ \hline 
 5 & 34317 & 1753783 & 4159210 & 65272.42 & 261.82 & -3.50 & 0.97247 & 5 & 35787 & 1782201 & 4744044 & 74677.50 & 145.76 & -3.50 & 0.54247 \\ \hline 
\end{tabular}


==> tables3/garver6Zhang2013HV_branch.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}\hline
   & fbus & tbus &   r  &   x  &   b  &  rateA &  rateB &  rateC \\ \hline 
   & 1.00 & 2.00 & 0.04 & 0.40 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 2.00 & 0.04 & 0.40 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 2.00 & 0.01 & 0.10 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 3.00 & 0.04 & 0.38 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 3.00 & 0.04 & 0.38 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 3.00 & 0.01 & 0.10 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 4.00 & 0.06 & 0.60 & 0.00 &  80.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 4.00 & 0.06 & 0.60 & 0.00 &  80.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 4.00 & 0.01 & 0.15 & 0.00 & 160.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 5.00 & 0.02 & 0.20 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 5.00 & 0.02 & 0.20 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 5.00 & 0.01 & 0.05 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 6.00 & 0.07 & 0.68 & 0.00 &  70.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 6.00 & 0.07 & 0.68 & 0.00 &  70.00 & 250.00 & 250.00 \\ \hline 
   & 1.00 & 6.00 & 0.02 & 0.17 & 0.00 & 140.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 3.00 & 0.02 & 0.20 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 3.00 & 0.02 & 0.20 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 3.00 & 0.01 & 0.05 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 4.00 & 0.04 & 0.40 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 4.00 & 0.04 & 0.40 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 4.00 & 0.01 & 0.10 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 5.00 & 0.03 & 0.31 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 5.00 & 0.03 & 0.31 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 5.00 & 0.02 & 0.16 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 6.00 & 0.03 & 0.30 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 6.00 & 0.03 & 0.30 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 2.00 & 6.00 & 0.01 & 0.08 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 4.00 & 0.06 & 0.59 & 0.00 &  82.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 4.00 & 0.06 & 0.59 & 0.00 &  82.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 4.00 & 0.01 & 0.15 & 0.00 & 164.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 5.00 & 0.02 & 0.20 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 5.00 & 0.02 & 0.20 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 5.00 & 0.01 & 0.05 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 6.00 & 0.05 & 0.48 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 6.00 & 0.05 & 0.48 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 3.00 & 6.00 & 0.01 & 0.12 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 4.00 & 5.00 & 0.06 & 0.63 & 0.00 &  75.00 & 250.00 & 250.00 \\ \hline 
   & 4.00 & 5.00 & 0.06 & 0.63 & 0.00 &  75.00 & 250.00 & 250.00 \\ \hline 
   & 4.00 & 5.00 & 0.02 & 0.16 & 0.00 & 150.00 & 250.00 & 250.00 \\ \hline 
   & 4.00 & 6.00 & 0.03 & 0.30 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 4.00 & 6.00 & 0.03 & 0.30 & 0.00 & 100.00 & 250.00 & 250.00 \\ \hline 
   & 4.00 & 6.00 & 0.01 & 0.08 & 0.00 & 200.00 & 250.00 & 250.00 \\ \hline 
   & 5.00 & 6.00 & 0.06 & 0.61 & 0.00 &  78.00 & 250.00 & 250.00 \\ \hline 
   & 5.00 & 6.00 & 0.06 & 0.61 & 0.00 &  78.00 & 250.00 & 250.00 \\ \hline 
   & 5.00 & 6.00 & 0.01 & 0.15 & 0.00 & 156.00 & 250.00 & 250.00 \\ \hline 
\end{tabular}


==> tables3/garver6Zhang2013HV_bus.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
   &  bus & type &   Pd   &   Qd  &  Gs  &  Bs  & area &  Vm  &  Va  & baseKV & zone & Vmax & Vmin \\ \hline 
   & 1.00 & 3.00 & 240.00 & 48.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 230.00 & 1.00 & 1.05 & 1.00 \\ \hline 
   & 2.00 & 1.00 & 240.00 & 48.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 230.00 & 1.00 & 1.05 & 1.00 \\ \hline 
   & 3.00 & 2.00 &  40.00 &  8.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 230.00 & 1.00 & 1.05 & 1.00 \\ \hline 
   & 4.00 & 1.00 & 160.00 & 32.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 230.00 & 1.00 & 1.05 & 1.00 \\ \hline 
   & 5.00 & 1.00 & 240.00 & 48.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 230.00 & 1.00 & 1.05 & 1.00 \\ \hline 
   & 6.00 & 2.00 &  0.00  &  0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 230.00 & 1.00 & 1.05 & 1.00 \\ \hline 
\end{tabular}


==> tables3/garver6Zhang2013HV_gen.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
   &  bus &  Pg  &  Qg  &  Qmax  &  Qmin  &  Vg  &  mBase & status &  Pmax  & Pmin &  Pc1 &  Pc2 & Qc1min & Qc1max & Qc2min & Qc2max \\ \hline 
   & 1.00 & 0.00 & 0.00 &  0.00  &  0.00  & 1.00 & 100.00 &  1.00  &  0.00  & 0.00 & 0.00 & 0.00 &  0.00  &  0.00  &  0.00  &  0.00  \\ \hline 
   & 3.00 & 0.00 & 0.00 & 150.00 & -10.00 & 1.00 & 100.00 &  1.00  & 360.00 & 0.00 & 0.00 & 0.00 &  0.00  &  0.00  &  0.00  &  0.00  \\ \hline 
   & 6.00 & 0.00 & 0.00 & 200.00 & -10.00 & 1.00 & 100.00 &  1.00  & 610.00 & 0.00 & 0.00 & 0.00 &  0.00  &  0.00  &  0.00  &  0.00  \\ \hline 
\end{tabular}


==> tables3/garver6Zhang2013HV_m1_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             & DC VM &  VA  &  PWL1 VM  &  VA  &  PWL2 VM  &  VA  & IPM VM &  VA  & SDP VM &  VA  \\ \hline 
   Obj / T   &  0.00 & 0.03 & 467276.00 & 0.18 & 466412.00 & 1.33 &  0.00  & 0.08 &  0.00  & 2.15 \\ \hline 
 RMSE / MAPE &  0.11 & 0.03 &    1.33   & 0.31 &    1.34   & 0.31 &  0.00  & 0.00 &  0.43  & 0.31 \\ \hline 
      B1     &  1.00 & 0.00 &    1.00   & 0.00 &    1.00   & 0.00 &  1.01  & 0.00 &  0.40  & 0.00 \\ \hline 
      B2     &  1.00 & 0.98 &    1.00   & 0.27 &    1.00   & 0.27 &  1.01  & 0.94 &  0.41  & 0.95 \\ \hline 
      B3     &  1.00 & 3.13 &    1.01   & 0.83 &    1.00   & 0.84 &  1.03  & 2.90 &  0.41  & 2.94 \\ \hline 
      B4     &  1.00 & 1.11 &    1.00   & 0.30 &    1.00   & 0.29 &  1.02  & 1.08 &  0.41  & 1.10 \\ \hline 
      B5     &  1.00 & 0.41 &    1.00   & 0.11 &    1.00   & 0.11 &  1.01  & 0.39 &  0.40  & 0.40 \\ \hline 
      B6     &  1.00 & 5.85 &    1.01   & 1.57 &    1.01   & 1.55 &  1.04  & 5.56 &  0.42  & 5.54 \\ \hline 
\end{tabular}


==> tables3/garver6Zhang2013HV_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             &   DC VM   &  VA  &  PWL1 VM  &  VA  &  PWL2 VM  &  VA  &   IPM VM  &  VA  &   SDP VM  &  VA  \\ \hline 
   Obj / T   & 465600.00 & 0.08 & 467276.00 & 0.11 & 466412.00 & 0.48 & 469456.78 & 0.09 & 469456.78 & 2.69 \\ \hline 
 RMSE / MAPE &    0.16   & 0.05 &    1.27   & 0.31 &    1.27   & 0.31 &    0.00   & 0.00 &    0.00   & 0.00 \\ \hline 
      B1     &    1.00   & 0.00 &    1.00   & 0.00 &    1.00   & 0.00 &    1.02   & 0.00 &    1.02   & 0.00 \\ \hline 
      B2     &    1.00   & 0.98 &    1.00   & 0.27 &    1.00   & 0.27 &    1.03   & 0.91 &    1.03   & 0.91 \\ \hline 
      B3     &    1.00   & 3.16 &    1.01   & 0.83 &    1.00   & 0.84 &    1.05   & 2.86 &    1.05   & 2.86 \\ \hline 
      B4     &    1.00   & 1.10 &    1.00   & 0.30 &    1.00   & 0.29 &    1.03   & 1.03 &    1.03   & 1.03 \\ \hline 
      B5     &    1.00   & 0.41 &    1.00   & 0.11 &    1.00   & 0.11 &    1.03   & 0.38 &    1.03   & 0.38 \\ \hline 
      B6     &    1.00   & 5.81 &    1.01   & 1.57 &    1.01   & 1.55 &    1.05   & 5.34 &    1.05   & 5.34 \\ \hline 
\end{tabular}


==> tables3/garver6y_000_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             & DC VM &  VA  & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &  VA  \\ \hline 
   Obj / T   &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
 RMSE / MAPE &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B1     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B2     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B3     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B4     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B5     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B6     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
\end{tabular}


==> tables3/garver6y_001_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             &  DC VM  &   VA   & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &  VA  \\ \hline 
   Obj / T   & 1840.00 &  0.75  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
 RMSE / MAPE &   6.67  &  1.99  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B1     &   1.00  &  0.00  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B2     &   1.00  &  6.11  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B3     &   1.00  &  7.64  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B4     &   1.00  & -18.33 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B5     &   1.00  &  -3.06 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B6     &   1.00  &  37.05 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
\end{tabular}


==> tables3/garver6y_010_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             & DC VM &  VA  & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &  VA  \\ \hline 
   Obj / T   &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
 RMSE / MAPE &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B1     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B2     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B3     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B4     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B5     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B6     &  0.00 & 0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
\end{tabular}


==> tables3/garver6y_011_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             &  DC VM  &   VA  & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &  VA  \\ \hline 
   Obj / T   & 1360.00 &  0.04 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
 RMSE / MAPE &   9.78  &  1.27 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B1     &   1.00  &  0.00 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B2     &   1.00  & -7.78 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B3     &   1.00  &  1.55 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B4     &   1.00  & 20.78 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B5     &   1.00  & -6.10 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B6     &   1.00  & 36.60 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
\end{tabular}


==> tables3/garver6y_100_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             &  DC VM  &   VA   & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &  VA  \\ \hline 
   Obj / T   & 1840.00 &  0.03  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
 RMSE / MAPE &   6.67  &  1.99  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B1     &   1.00  &  0.00  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B2     &   1.00  &  6.11  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B3     &   1.00  &  7.64  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B4     &   1.00  & -18.33 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B5     &   1.00  &  -3.06 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B6     &   1.00  &  37.05 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
\end{tabular}


==> tables3/garver6y_110_table.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}\hline
             &  DC VM  &   VA   & PWL1 VM &  VA  & PWL2 VM &  VA  & IPM VM &  VA  & SDP VM &  VA  \\ \hline 
   Obj / T   & 1412.22 &  0.03  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
 RMSE / MAPE &   7.85  &  -1.29 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B1     &   1.00  &  0.00  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B2     &   1.00  &  6.11  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B3     &   1.00  &  7.64  &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B4     &   1.00  & -18.33 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B5     &   1.00  &  -3.06 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
      B6     &   1.00  &  37.05 &   0.00  & 0.00 &   0.00  & 0.00 &  0.00  & 0.00 &  0.00  & 0.00 \\ \hline 
\end{tabular}


==> tables3/garver6y_111_branch.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
   & fbus & tbus &   r  &   x  &   b  &  rateA &  rateB &  rateC & ratio & angle & status &  angmin & angmax \\ \hline 
   & 1.00 & 2.00 & 0.04 & 0.40 & 0.00 & 180.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
   & 1.00 & 4.00 & 0.06 & 0.60 & 0.00 & 150.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
   & 1.00 & 5.00 & 0.01 & 0.10 & 0.00 & 360.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
   & 2.00 & 3.00 & 0.02 & 0.20 & 0.00 & 180.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
   & 2.00 & 4.00 & 0.04 & 0.40 & 0.00 & 180.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
   & 2.00 & 6.00 & 0.01 & 0.15 & 0.00 & 360.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
   & 3.00 & 5.00 & 0.01 & 0.10 & 0.00 & 360.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
   & 3.00 & 6.00 & 0.02 & 0.24 & 0.00 & 360.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
   & 4.00 & 6.00 & 0.01 & 0.08 & 0.00 & 360.00 & 250.00 & 250.00 &  0.00 &  0.00 &  1.00  & -360.00 & 360.00 \\ \hline 
\end{tabular}


==> tables3/garver6y_111_bus.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
   &  bus & type &   Pd   &   Qd  &  Gs  &  Bs  & area &  Vm  &  Va  & baseKV & zone & Vmax & Vmin \\ \hline 
   & 1.00 & 3.00 &  80.00 & 16.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 230.00 & 1.00 & 1.05 & 0.95 \\ \hline 
   & 2.00 & 1.00 & 240.00 & 48.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 230.00 & 1.00 & 1.05 & 0.95 \\ \hline 
   & 3.00 & 2.00 &  40.00 &  8.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 230.00 & 1.00 & 1.05 & 0.95 \\ \hline 
   & 4.00 & 1.00 & 160.00 & 32.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 230.00 & 1.00 & 1.05 & 0.95 \\ \hline 
   & 5.00 & 1.00 & 240.00 & 48.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 230.00 & 1.00 & 1.05 & 0.95 \\ \hline 
   & 6.00 & 2.00 &  0.00  &  0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 230.00 & 1.00 & 1.05 & 0.95 \\ \hline 
\end{tabular}


==> tables3/garver6y_111_gen.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
   &  bus &  Pg  &  Qg  &  Qmax  &  Qmin  &  Vg  &  mBase & status &  Pmax  & Pmin &  Pc1 &  Pc2 & Qc1min & Qc1max & Qc2min & Qc2max \\ \hline 
   & 1.00 & 0.00 & 0.00 &  48.25 & -10.00 & 1.00 & 100.00 &  1.00  & 160.00 & 0.00 & 0.00 & 0.00 &  0.00  &  0.00  &  0.00  &  0.00  \\ \hline 
   & 3.00 & 0.00 & 0.00 & 101.25 & -10.00 & 1.00 & 100.00 &  1.00  & 370.00 & 0.00 & 0.00 & 0.00 &  0.00  &  0.00  &  0.00  &  0.00  \\ \hline 
   & 6.00 & 0.00 & 0.00 & 183.00 & -10.00 & 1.00 & 100.00 &  1.00  & 610.00 & 0.00 & 0.00 & 0.00 &  0.00  &  0.00  &  0.00  &  0.00  \\ \hline 
\end{tabular}

